Visual Evaluation of Generative Adversarial Networks for Time Series Data

A crucial factor to trust Machine Learning (ML) algorithm decisions is a good representation of its application field by the training dataset. This is particularly true when parts of the training data have been artificially generated to overcome common training problems such as lack of data or imbalanced dataset. Over the last few years, Generative Adversarial Networks (GANs) have shown remarkable results in generating realistic data. However, this ML approach lacks an objective function to evaluate the quality of the generated data. Numerous GAN applications focus on generating image data mostly because they can be easily evaluated by a human eye. Less efforts have been made to generate time series data. Assessing their quality is more complicated, particularly for technical data. In this paper, we propose a human-centered approach supporting a ML or domain expert to accomplish this task using Visual Analytics (VA) techniques. The presented approach consists of two views, namely a GAN Iteration View showing similarity metrics between real and generated data over the iterations of the generation process and a Detailed Comparative View equipped with different time series visualizations such as TimeHistograms, to compare the generated data at different iteration steps. Starting from the GAN Iteration View, the user can choose suitable iteration steps for detailed inspection. We evaluate our approach with a usage scenario that enabled an efficient comparison of two different GAN models.

==> content/0-abstract.tex <==
\abstract{
Over the last few years, Generative Adversarial Networks (GANs) have shown remarkable results in
generating realistic data. Machine Learning (ML) experts use this technique %to generate new data based on existing ones 
to deal with common training problems such as lack of data or imbalanced dataset. % with the aim of 
%\textbf{Which data? Training data for ML? Evaluation data?}. 
However,
this ML approach lacks an objective function to evaluate the quality of the generated data. 
Also, most evaluation methods are designed specifically for image models and can not be easily applied to time series data.
In this paper, we present a Visual Analytics (VA) approach
to evaluate the performance of GAN for time series data. The presented approach consists of two views, namely a GAN Iteration View showing similarity metrics per time series over the iterations of the generation process and a Detailed Comparative View equipped with compact time series visualizations and TimeHistograms%[and Colorfields] \textbf{Colorfields sind doch eine "compact TS visualization"? Ich wuerde colorfields weglassen}
, to compare the generated data at different iteration steps by juxtaposition.
%highlighting the time series and the corresponding distributions.
Starting from the GAN Iteration View, the user can choose suitable iteration steps for detailed inspection.
%Starting from an aggregated view showing similarity metrics per time series over the iterations of the generation process, the user can choose suitable iterations for detailed inspection.
%Compact time-series visualizations are used to compare the generated data at different iteration steps by juxtaposition. ML 
We evaluate our approach with a usage scenario that enabled an efficient comparison of two different GAN models.
%We evaluate our approach by demonstrating which model is the right onemodels
}

